Tracking Summer Greenland Blocking: the Upstream Pathway Shapes Historical Extremes and Future Change

The representation and future evolution of summer Greenland atmospheric blocking in climate models is here investigated from a Lagrangian perspective using a novel Python package blocktrack. By applying the blocktrack algorithm to ERA5 reanalysis and a CMIP6 model ensemble, we identify and track blocking events over Greenland, and obtain their trajectories, intensities, duration and wave-breaking patterns. Greenland blocking (GB) events in ERA5 are then classified into two types based on their wave-breaking characteristics. These correspond to the previously identified upstream (anticyclonic wave breaking) and retrograding (cyclonic wave breaking) GBs. Upstream blocks, which originate in Northern Canada, exhibit stronger moisture transport before and during blocking onset and higher temperature anomalies than retrograding blocks, which follow an east-to-west trajectory and originate in the North Atlantic. Our analyses show how the recent observed increase in GB frequency, particularly in 2012, is primarily driven by upstream blocks. CMIP6 models generally fail to capture the observed increase and underestimate GB variability, especially for the upstream component. Projections under the SSP3-7.0 scenario show a decline in retrograding blocks but a possible increase in upstream blocks, depending on the detection index used. We discuss possible drivers of these changes, which include jet stream shifts, increased frequency of high-moisture transport events from low to high latitudes, surface temperature increases due to Atlantic Multidecadal Variability and Arctic Amplification. By analyzing block trajectories, this study demonstrates how Lagrangian diagnostics can provide novel insights into the dynamics of blocking events over Greenland.

==> correlations_table.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|} \hline 
         /&  GHA&  GHA upstream& GHA retrograding\\ \hline 
         DAV&  0.20&  0.11& 0.15\\ \hline 
         DAV upstream&  0.11&  0.12& 0.05\\ \hline 
         DAV retrograding&  0.13&  0.05& 0.15\\ \hline
    \end{tabular}
    \caption{Jaccard coefficients for the Boolean time-series produced through the DAV and GHA indices. GHA and DAV refer to the time series of blocked and non-blocked days in the Greenland region, the suffix 'upstream' refers to the time-series where only upstream blocks are retained and the suffix 'retrograding' refers to the time-series where only retrograding blocks are retained. For the details on how the coefficient has been computed see the Methods section.}
    \label{jaccard}
\end{table}

In Table \ref{jaccard} we show the Jaccard coefficient of the boolean time series obtained through the different blocking indices. It is evident how the coefficients assume very small values for all the combination (1 = highly correlated, 0 = uncorrelated). This low correlation is motivated by the fact that blocking occurs rarely and when it occurs the different indices identify blockings in different areas and at different stages of its life-cycle. Yet, Table \ref{jaccard} contains some useful information. In order to confirm that such correlations are not random we note that the combinations (GHA upstream, DAV retrograding) and (GHA retrograding, DAV upstream) are very little correlated, as expected. Moreover, it is possible to notice that the maximum correlation are obtained when considering all the events (DAV, GHA) or when considering the retrograding events (DAV retrograding, GHA retrograding), while the upstream events are less correlated. This further sustain the idea that upstream events are Omega blocks that can develop into Rex blocks. The GHA index struggles with detecting Rex blocks and the intrusion of polar air from higher latitudes, while the DAV index struggles with detecting Omega blocks, resulting in a weaker correlation between the two. Conversely, retrograding blocks consist in breaking Rossby waves that can be effectively detected by both indices, resulting in a slightly higher correlation.

